Egorov property in perturbed cat map

We study the time evolution of the quantum-classical correspondence (QCC) for the well known model of quantised perturbed cat maps on the torus in the very specific regime of semi-classically small perturbations. The quality of the QCC is measured by the overlap of classical phase-space density and corresponding Wigner function of the quantum system called quantum-classical fidelity (QCF). In the analysed regime the QCF strongly deviates from the known general behaviour in particular it decays faster then exponential. Here we study and explain the observed behavior of the QCF and the apparent violation of the QCC principle.

==> Makefile <==
FILE=egorov_doc

all: $(FILE).dvi

egorov_doc.dvi: $(FILE).tex *.eps
	latex $(FILE)
	latex $(FILE)

egorov_doc.ps: $(FILE).dvi
	dvips -Ppdf -G0 $(FILE)

egorov_doc.A4.ps: $(FILE).ps
	csh ~/scripts/psA4toA5 -duplex $(FILE).ps $(FILE).A4.ps
	
egorov_doc.pdf:egorov_doc.ps
	ps2pdf $(FILE).ps $(FILE).pdf


egorov_doc.djvu: $(FILE).ps
	djvudigital $(FILE).ps

# my shortcuts

ps: $(FILE).ps

ps.A4: $(FILE).A4.ps

pdf: $(FILE).pdf

djvu: $(FILE).djvu

archive:
	tar -cvzf $(FILE).tar.gz `bash search $(FILE).tex` \
	search iopart*.cl* Makefile

zip:
	zip $(FILE).zip `bash search $(FILE).tex` \
        search iopart*.cl* Makefile
clean:
	rm -f *~ $(FILE).dvi $(FILE).bbl $(FILE).log $(FILE).blg \
	$(FILE).aux $(FILE).ps $(FILE).A4.ps $(FILE).pdf $(FILE).tar.gz


==> search <==
#!/bin/bash

#
# The skripts searches recursively the .tex file and prints out the
# files that used in its creation 
#


#
# usage: sh search file.tex
#

########################################################################

# find_in_file(filename)
function find_in_file { 	

echo $1;

tmp=`cat $1 | sed -e 's/%.*//'`;

echo $tmp | sed -e 's/\\/\n/g'| while read line; do

  line=${line% }
  line=${line# }

  if [ -n "$line" ]; then

    if [ -z "${line%includegraphics*}" ]; then
      echo $line | sed 's/includegraphics[^{]*{\([^}]*\)}.*/\1/';
    elif [ -z "${line%include*}" ]; then
      filename=`echo $line | sed 's/include[^{]*{\([^}]*\)}.*/\1/'`;
      find_in_file "${filename}.tex";
    elif [ -z "${line%input*}" ]; then
      filename=`echo $line | sed 's/input[^{]*{\([^}]*\)}.*/\1/'`;
      find_in_file "${filename}" ;   
    elif  [ -z "${line%bibliographystyle*}" ]; then
      echo `echo $line | sed 's/bibliographystyle[^{]*{\([^}]*\)}.*/\1/'`.bst;
    elif  [ -z "${line%bibliography*}" ]; then
      echo `echo $line | sed 's/bibliography[^{]*{\([^}]*\)}.*/\1/'`.bib;
    fi
  fi
done;

}

find_in_file $1 

